Reduction of Abelian Varieties and Grothendieck's Pairing

We prove that abelian varieties of small dimension over discrete valuated, stricty henselian ground fields with perfect residue class field obtain semistable reduction after a tamely ramified extension of the ground field. Using this result we obtain perfectness results for Grothendieck's pairing.

==> weil.tex <==
\section{Weil restriction}

We follow \cite{bb}, section 1. In the situation of the previous section let $R$ be a henselian
discrete valuation ring. We fix the following notation: Let $L/K$ be a finite Galois extension, $S$
the integral closure of $R$ in $L$, $l/k$ the residue class field extension. We write
\[
X_K\defeq\scrR_{L/K} A_L
\]
for the Weil restriction of the abelian variety $A_L\defeq A_K\times_K L$. It  is easy to see that
$X_R\defeq\scrR_{S/R} A_S$ is the associated Néron model. (Here $A_S$ is the Néron model of $A_L$.
In general it \emph{does not} hold that $A_S=A_R\times_R S$).  By $\oldphi_{X_R}$, $\oldphi_{A_S}$
etc.\ we denote the corresponding groups of components.
\par
In this situation we have the following proposition:


\begin{prop}\label{weil_phi_iso}
The canonical morphism $X_R\times_R S\to A_S$ induces a morphism
\[
\oldphi_{X_R}\times_k l\longto\oldphi_{A_S}.
\]
If $l/k$ is purely inseperable, this is an isomorphism.
\end{prop}

\begin{proof}
\cite{bb}, proposition 1.1.
\end{proof}

From now on, we assume $R$ to be a strictly henselian discrete valuation ring with perfect, i.\,e.\
algebraically closed residue class field of characteristic $p\neq 0$. Then every finite extension
of $k$ is purely inseparable (namely trivial) and we can identify $\oldphi_{A_S}$ and
$\oldphi_{X_R}$ by means of this proposition. 
\par
In this situation, we can allow a tamely ramified
extension of $K$ to test whether or not Grothendieck's pairing is perfect:

\begin{prop}\label{gp_perf_tamely}
Let $R$ be as stated above and let $L/K$ be a tamely ramified Galois extension. Consider the followind
assertions.
\begin{enumprop}
  \item Grothendieck's pairing for $A_S$ and $A'_S$ is perfect.
  \item Grothendieck's pairing for $X_R$ and $X'_R$ is perfect.
  \item Grothendieck's pairing for $A_R$ and $A'_R$ is perfect.
\end{enumprop}
Then we have $\enum 1\iff\enum 2\then\enum 3$.
\end{prop}

We give a short review of the proof as given in \cite{bb}, Corollary 3.1:

\begin{proof}
Let $n\defeq[L:K]$. Then $p$ does not divide $n$. As shown in \cite{bb}, Lemma 2.2 we have
the following equality:
\[
[n]\circ \gp_{X_R}=[n]\circ\gp_{A_S},
\]
where $[n]$ denotes the $n$-multiplication on the appropriate group of components. It follows that
the kernels of both compositions coincide (after identification as in proposition
\ref{weil_phi_iso}). Since $\gp$ is an isomorphism on the prime-to-$p$-part and $n$ is prime to
$p$, the kernels of $\gp_{X_R}$ and $\gp_{A_S}$ coincide. This shows the equivalence of \enum 1 and
\enum 2.
\par
As in the proof of \cite{bb}, corollary 3.1 we have two morphisms
\[
A_R\longto X_R\longto A_R,
\]
such that their compositions is the multiplication with $n$. These morphisms induce morphisms on
the schemes, representing $\sext^1(-,\bbG_m)$ and their component groups.  If we keep in mind the
equality $\ker\gp_{A_R}=\pi_0\sext^1(A_R,\bbG_m)$, we have two morphisms
\[
\ker\gp_{A_R}\longto  \ker\gp_{X_R}\longto \ker\gp_{A_R},
\]
such that the composition is the multiplication by $n$. As these groups are $p$-groups
(proposition \ref{gp_diag}) and $p$ is prime to $n$, the first morphism is injective, hence \impl 2 3.
\end{proof}

The following result is due to \cite{ell}, Theorem 1:


\begin{cor}\label{ker_killed}
Let $R$ be as above and let $L/K$ be any Galois extension of degree $n$.
\begin{enumprop}
  \item The kernel of the map $\gamma_{L/R}\colon\oldphi_{A_R}\to\oldphi_{A_S}$ is killed by $n$.
  \item Let $n=p_1^{e_1}\cdot\ldots\cdot p_n^{e_n}$.be the prime decomposition of $n$ and $\ell$ a prime
    different from $p_1,\ldots,p_n$. Then $\gamma$ restricts to an injection
    \[
    \oldphi_{A_R,\ell}\longinto\oldphi_{A_S,\ell}.
    \]
\end{enumprop}
\end{cor}


\begin{proof}
As in the above proof, we have two morphisms $A_R\to X_R\to A_R$, such
that their composition is the multiplication with $n$. They induce maps of the component groups
$\oldphi_{A_R}$ and $\oldphi_{X_R}\iso\oldphi_{A_S}$ with the same property. Consequently, we have
$\ker\gamma_{L/R}\sub\ker[n]$. 
\end{proof}


